iNNk: A Multi-Player Game to Deceive a Neural Network

This paper presents iNNK, a multiplayer drawing game where human players team up against an NN. The players need to successfully communicate a secret code word to each other through drawings, without being deciphered by the NN. With this game, we aim to foster a playful environment where players can, in a small way, go from passive consumers of NN applications to creative thinkers and critical challengers.

==> holdtext.tex <==
%AI and its impact on game design - overview
%Classic AI research in games focus on creating AI agents that can compete with human players. Recently, research efforts have shifted to use AI to improve player experience \cite{riedl2013ai,yannakakis2018artificial}. 

%\section{Discussion}
%\textcolor{red}{JV: Perhaps we can discuss, for future work, how we intend to balance the gameplay between humans and the NN. Once a player knows a strategy works (i.e.,cross hatching), this would make the game very easy moving forward and players may exploit this strategy. We can discuss directions to consider that may help correct this issue and ways to limit the player to encourage new thinking/strategies. We can highlight specifics, such as limiting ink the next round when cross-hatching is being detected, but we do not yet address the more creative strategies such as drawing socially Also, the same can be said for the NN being too good at guessing. How do we intend to limit the NN in the case players are not thinking of new strategies?}

Previous drafts

%iNNk is a round-based multiplayer drawing game where two or more humans team up to communicate a secret code word before the NN can interpret it. Players in the Human Team cycle through two roles: Sketcher, the one who illustrates the code word, and Guesser, the one(s) who interpret(s) the illustration to guess the code word. These roles are randomly set at the beginning of each round. The NN always behaves like a Guesser, trying to figure out the code word before the human player(s).

%The game is played in a series of 30-second rounds, the overall winner being the team that wins the best out of five rounds. When human players or the NN correctly guesses a word, the round ends, and the respective team wins a point. If the round ends without a team correctly guessing the word, no one earns a point, and the round is repeated with a new word. Incorrect guesses, including the NN’s, are shown to the right of the screen while the round is active. 

%{\color{magenta} Our NN's training data, from \emph{Quick, Draw!}, is drawn in under 20 seconds. To keep the source of our NN's dataset uses 20 second rounds but we added extra time to account for the multiplayer aspect of our game. 30-second rounds provides quick bursts of action}

%We chose 30-second rounds because of their quick bursts of action. As the Sketcher’s drawing becomes more detailed, the pressure grows on the Guesser(s) and the NN to correctly guess the code word first. This fast paced cycle allows players to quickly change and experiment with their drawings.


%\subsection{Design Intent}
%We set off to explore how NNs that are embedded into the core gameplay loop inspire new player-NN interactions in a multiplayer, team-based game. Our Design Goal is to provide a fun and accessible gameplay experience that increases players’ familiarity of Deep Learning/ Neural Networks, specifically its output confidence accuracy (ie. how sure it is when making a guess).


%These strategies are very interesting. But we need to tie it more to our design goal and why these strategies indicate a good gameplay experience. As is, this shows how players can trick the NN and win the game. But that's not necessarily a fun game because then you will almost always win. Can you write more about how in each player strategy, the game provides a fun player experience

\subsection{Features and Aesthetics}
%iNNk aims to provide a fun and accessible gameplay experience through two main features. First, we present the NN as a system and reveal the certainty of its guesses through a Confidence Meter. Second, we create an adversarial game setting where the player's opponent is the NN, creating a consistent reminder of the underlying system. Together these two features create tension for the players, highlighting a key feature of the NN - that it is not always confident in the accuracy of the output it provides.

%The NN is an opponent to the human players, directly counteracting their efforts to win the game. Its presence creates tension through its facial expression and monitor color. Additionally, there are two design choices that add to the tension: the score is presented as Human Players vs NN and the NN’s guesses are placed above the human players’ to the right of the screen.

%The Confidence Meter is the NN’s certainty in regards to its analysis of the Sketcher’s drawing. This UI element reveals how the NN analyzes the input and that it is not always certain of its output’s accuracy. A common assumption is that a system is always accurate or correct in its output; however, that is not the case. With this design feature, our goal is to familiarize players with how deep learning works in a fun and accessible way.

%Additionally, the Confidence Meter acts as a secondary timer for the players, letting them know when the NN is close to making a guess and possibly winning a round. This creates a steady increase in engagement within each round. This encourages Guessers to think quickly about the Sketcher’s drawing, while the Sketchers think broadly about drawing in ways that the NN won’t understand. 

%The game is designed to be fun by surprising the players when they lose to the NN and realize that it can understand drawings like humans can. Players have to collaborate creatively when figuring out ways to deceive the NN.

%\subsection{Player Strategies}
%These strategies are very interesting. But we need to tie it more to our design goal and why these strategies indicate a good gameplay experience. As is, this shows how players can trick the NN and win the game. But that's not necessarily a fun game because then you will almost always win. Can you write more about how in each player strategy, the game provides a fun player experience

%We intend to increase the player's familiarity with Deep Learning by encouraging players to try new drawing strategies through the features mentioned above. The experience is designed so that players can quickly observe the correlation between their drawing and the NN’s confidence meter, allowing them to observe the effects of any experimentation in real time. Three of the most common strategies players experiment with are pictograms/ rebus puzzles, less common interpretations of the word, and creating noise/distractions around the drawing board.

%Pictograms are a clever way of illustrating compound words! For example, if the Sketcher is given the word eyeglasses they would be able to draw an eye and a pair of drinking glasses. Humans are able to put eye and glasses together to get the compound word eyeglasses, but the NN would not be able to. For non-compound words it can be a little harder, but it is still possible. If the Sketcher were to draw a bee and then add some rain, a Guesser could understand that the answer is the word brain.

%Some words can have multiple meanings, some more common than others. These words are special because the NN might not be familiar with less common definitions. Some easy ones are, for example, drawing a computer mouse instead of the animal mouse or drawing a hammer’s nail instead of a fingernail. All four are technically correct, but the NN will have an easier time identifying some drawings over others.

%The final common strategy for tricking the NN is creating noise and distractions around or on top of the drawing. Humans are able to parse out what is and isn't nonsense, but the NN cannot. If the Sketcher were to hatch over the drawing area, the NN would take those strokes at face value and try to analyze them. It will take longer for the NN to correctly identify the code word, if it is still even possible. 
